Negation-Closure for JSON Schema

JSON Schema is an evolving standard for describing families of JSON documents. It is a logical language, based on a set of assertions that describe features of the JSON value under analysis and on logical or structural combinators for these assertions, including a negation operator. Most logical languages with negation enjoy negation closure, that is, for every operator they have a negation dual that expresses its negation. We show that this is not the case for JSON Schema, we study how that changed with the latest versions of the Draft, and we discuss how the language may be enriched accordingly. In the process, we define an algebraic reformulation of JSON Schema, which we successfully employed in a prototype system for generating schema witnesses.

==> jsonschema.tex <==
% !TeX root = main_vldb.tex


%\hide{


%\begin{definition}[Value equality and sets of values] In the following we denote value equality with the usual notation $\J_1 = \J_2$, with the expected meaning on base values, while on objects we have that  $O_1 = O_2$ iff $O_1= \{l_1:\J_1,\ldots,l_n:\J_n \}$ and  $O_2= \{l_{\pi(1)}:\J'_{\pi(1)},\ldots,l_{\pi(n)}:\J'_{\pi(n)} \}$ with $\pi$ a permutation over $I=\SetTo{n}$ and $\J_i=\J'_{\pi(i)}$ for each $i\in I $. On arrays we have  $A_1 = A_2$  iff $ A_1 = [\J_1, \ldots, \J_n ] $ and $A_2 = [\J'_1, \ldots, \J'_n ] $ with $J_i = J'_i$ for each $i\in \SetTo{n}$.
%
%Sets of {\json}  values are %defined as 
%unordered collections without repetitions w.r.t.\ this notion of equality.
%
%\end{definition}

%The order of object members is irrelevant, that is
%$\{l_1:\J_1,\ldots,l_n:\J_n \} = \{l_{\pi(1)}:\J_{\pi(1)},\ldots,l_{\pi(n)}:\J_{\pi(n)} \}$, when $\pi$ is a permutation.

%, the order of object members is irrelevant.

\begin{toappendix}

\subsection{{\jsonsch} by example}\label{sec:jschema}

{\jsonsch} is a logical language whose terms are expressed as {\json} terms, and describe sets
of {\json} terms. 
%When discussing this schema, it will become apparent that
%the interaction of different operators, positioned in different lines in the document,
%can make programmatic processing and reasoning a challenge.

\begin{figure}[th]
\centering

\begin{Verbatim}[fontsize=\footnotesize,numbers=left,xleftmargin=0mm,numbersep=3pt,frame=lines]
{ "properties" : { "VAL" : { "type" : "number" },
                   "NEXTOBJ" :  { "type" : "object"  } },
  "patternProperties" : { "^NEXT" :  { "$ref" : "#" }, 
                          "STRING$" : { "type" : "string" } },
  "additionalProperties" : { "$ref" : "#/definitions/OBJROOT" },
  "required" : ["VAL", "NEEDED"],
  "minimum" : 1, 
  "definitions" : { "OBJROOT" : { "allOf" : [{ "$ref" : "#" }, 
                                             { "type" : "object"}]}}
}
\end{Verbatim}
\caption{A {\jsonsch} document.}
\label{fig:schema_example1}
\end{figure}

As an example, consider the document of Figure \ref{fig:schema_example1}. 
We use here \emph{schema} to indicate a subterm of a {\jsonsch} document that is either
an object or a boolean and that is used to validate instances. 
%In the above example, the outermost
%object is a schema, and all objects whose names are in small letters are schemas, while, for example,
%the value of the \xprops\ member is not a schema but is a set of pairs name-schema used as a parameter
%for the \xprops\ keyword.
Any {\jsonsch} document is a schema, which usually contains many nested schemas.
The members of a schema whose name is chosen among the \emph{assertion keywords} are called
\emph{assertions}, and here we have five of them at the outermost level: 
 \xprops, \xpattProps, \xaddProps, \xreq, and finally \xmin. A set of assertions collected inside a schema denotes a conjunction: an instance must satisfy all those assertions
to satisfy the schema.

\xdefs\ is not an assertion keyword. It is just a placeholder, which does not assert anything about the 
{\json} instance, but whose value contains a set of name-schema pairs: here, it is used
to associate the name \emph{OBJROOT} with the schema ``\{ \xast{\xall} : [...] \}''.\DC{rephrased a bit for better readability}


{\json} values belong to one of the six {\json} types: \xnumber, \xnull, \xboolean, \xstr, \xobject, \xarray.
All assertions that analyze the values of a specific type $T$ are \emph{conditional} on $T$, that is, their definition
is ``\emph{if} the instance belongs to $T$ \emph{then}\ldots'', so that every instance that does \emph{not}
belong to $T$ satisfies that assertion. For example, the \xprops\ assertion in line~1 
specifies that, if the instance is an object, then if the instance has a \emph{VAL} member, then its value is a number,
and, if it has a \emph{NEXTOBJ} field, then its value is an object. This assertion is conditional on the type {\qobject}, and 
hence it is satisfied by anything that is not an object, and is conditional on the presence of the members
\emph{VAL} and \emph{NEXTOBJ}, and hence it is satisfied
by any object without those members. 

The \xreq\ assertion forces the presence of the listed members, 
but is itself conditional on the type. %\footnote{%Observe that 
The fields listed in the \xprops\ assertions and those that 
are listed by \xreq\ are, in principle, not related: in the example, we restrict the value of \emph{NEXTOBJ} without forcing
its presence, and we require the \emph{NEEDED} field without restricting its value. %} 

\xpattProps\ specifies that, \emph{if} the instance is an object and \emph{if} a field name matches some pattern,
then the member value must satisfy the corresponding schema. {\jsonsch} patterns are 
matched against any substring of the target string unless they are anchored 
to the beginning of the target (using ``\NN'' as in ``\NN NEXT'') or to the end (using ``\$''
as in ``STRING\$'').
Hence, any member whose name begins with \emph{NEXT} must satisfy the assertion \mbox{``\{ \qdref  : \qkw{\#} \}''}
(to be discussed later)
and any member whose name ends in \emph{STRING} must satisfy the assertion ``\{ \qtype : \qstr \}''.
Hence, a member named \emph{NEXTxxxSTRING} must satisfy both, and a member named
\emph{NEXTOBJ} must satisfy both the schema ``\{ \qtype : \qobject    \}'' associated with  \emph{NEXTOBJ}
and the schema ``\{ \qdref  : \qkw{\#} \}''.%, since \xprops\ and \xpattProps\ are here connected by a conjunction.

\xaddProps\ is context-dependent: \emph{if} the instance is an object, if a member name
does not match any \xprops\ or \xpattProps\ that co-occur at the top level of the schema where \xaddProps\ occurs,
then the member value must satisfy the schema of \xaddProps.

\qmin\ : \kw{1} is a conditional assertion about numbers, meaning: if the instance is a number, then its minimum value
is 1. The combination of this assertion with the previous assertions, that are all conditional on the object types, 
means that: if the instance is a number, it must satisfy \qmin\ : \kw{1}. If it is an object, it must satisfy the other constraints
described. If it has any other type (\xnull, \xboolean, \xstr, \xarray), then it satisfies this schema.

A reference assertion \qdref  : \qkw{path} is a recursive reference, denoting a subschema (possibly also of a remote resource) reached by a path. Path ``\#'' denotes the root of the current document, while  
\qkw{\#/definitions/OBJROOT} is the schema that is the value of the \emph{OBJROOT} member of the \emph{definitions}
member of the root. This allows any subschema to refer to any other subschema.

Besides the conditional assertions, {\jsonsch} features boolean combinators such as \xall, for boolean
conjunction, \xany, for boolean disjunction, \xnot, for boolean negation, and others. 
For example, %the subschema 
\qall : [  \{ \qdref  : \qkw{\#} \} , \{ \qtype : \qobject  \} ] in the example requires
the instance to satisfy the root schema and to be an object, hence excluding all the other types.



%Reasoning about negation inside {\jsonsch} can be tricky, partly due to some elusive
%aspects of {\jsonsch} semantics, partly due to its non-algebraic nature. 
Figure~\ref{subfig:notrequired} is an example that contains the \xnot\ operator.
Lines~1 through~3 state which are the values allowed for \emph{color} and \emph{size} if the instance is an object
and if it contains those fields.
Line~4 actually declares that the instance \emph{must} be an object and \emph{must not} contain a property 
\verb!size!. This can be surprising for {\json} novices, since the assertion might be 
mistakenly read for a property not being required,
and therefore, \emph{optional}.%
\footnote{Note that this is not an artificially contrived example; for anecdotal evidence, 
we refer to  \emph{stackoverflow}:
\url{https://stackoverflow.com/questions/30515253/json-schema-valid-if-object-does-not-contain-a-particular-property}.}

Figure~\ref{subfig:notrequired_rewritten} shows an equivalent schema, 
where negation has been \emph{pushed down}, to the point of elimination. It is now explicit that property \verb!size! is not allowed (line~3).
Moreover, line~4 states that the schema allows only instances of type object (but not string constants, for example),
an assertion that was only implicit in the original schema.



\begin{figure}[bt]
 \centering
\begin{Verbatim}[fontsize=\small,numbers=left,numbersep=3pt,frame=lines,xleftmargin=5mm]
{ "properties": {
    "color": {"enum": ["white", "black"]},
    "size":  {"enum": ["S", "M", "L"]} },
  "not": {"required": ["size"]}
}
\end{Verbatim}
\caption{T-shirt schema with negation.}
\label{subfig:notrequired}
\end{figure}

\begin{figure}[bt]
 \centering
\begin{Verbatim}[fontsize=\small,numbers=left,numbersep=3pt,frame=lines,xleftmargin=5mm]
{ "properties": {
    "color": {"enum": ["white", "black"]},
    "size": false }, 
  "type": "object"
}
\end{Verbatim}
\caption{T-shirt schema after not-elimination.}
\label{subfig:notrequired_rewritten}
\end{figure}

\end{toappendix}

%This is just an informal description of the structure of  the language,
%and we refer to the official specification for details~\cite{Version09}. 
%The complete language is defined by all and only the operators that are listed in Figure~\ref{fig:reftrans}, 
%plus some other operators that we ignore since they are not related to validation, and hence do not impact the semantics that we
%describe here.

%%\begin{toappendix}
%\subsection{{\jsonsch} Drafts}\label{sec:study}
%
%At the time of writing, there are eight  versioned drafts of {\jsonsch}, the most recent being
%{\VerNine} \cite{Version09}. 
%We conducted an analysis of actual use of {\jsonsch},
%using Google BigQuery to crawl GitHub for {\jsonsch} files (as of July 2020), and retrieved over 91K
%documents. We found that {\VerFour} \cite{Draft04} is by far the most
%widely adopted, while  new features introduced by {\VerNine} did not appear in almost any of the schemas. 
%We thus formalize {\VerSix}~\cite{Draft06}, the last one before {\VerNine} 
%and a conservative extension of its predecessors.
%Indeed, it covers all collected schemas. However,
%{\VerNine} adds some features 
%that dramatically change the evaluation model. In particular, it adds operators 
%(\xmaxC\ and \xminC) that strongly impact negation closure, and, hence, we discuss them in Section~\ref{sec:mincontains}.
%%\end{toappendix}
%
%\hide{
%\begin{toappendix}
%\section{Versions of {\jsonsch}}
%
%To determine the current popularity of these versions, we conducted a large-scale analysis of real-world {\jsonsch} documents.
%Specifically, we used Google BigQuery\footnote{\url{https://cloud.google.com/bigquery/}}
%to identify {\jsonsch} documents hosted on GitHub,
%as of July 9th, 2020. 
%Google BigQuery is a commercial cloud service that allows for querying the 3TB+ GitHub open data collection, 
%comprising of mostly non-forked projects with an open source license. The data are refreshed weekly.
%
%We identified relevant documents by searching their content for the property \verb!$schema!, but excluding
%documents that specify the {\jsonsch} language itself (recognizable by the URL of the \verb!$id! property).
%This allowed us to identify over 91k unique URLs, some of which were no longer accessible.
%After download, duplicate-elimination, removal of schemas with syntax errors, 
%and reference expansion, we obtain
%approx.\  13,8k unique schemas.
% 
%We identified the draft version based on the URL in the \verb!$schema! property.
%%
%We found that  {\VerFour} \cite{Draft04} is the most widely used,
%dominating with 84\% among those which declare their version, 
%followed by {\VerSix}~\cite{Draft06} with 9\%. 
%The newest version, {\VerNine} \cite{Version09}, is not yet represented in the 91K schemas that we downloaded.
%
%%{\VerNine} \cite{Version09} is the latest but has some very peculiar features
%%as is not yet widely used, while the intermediate {\VerSix} \cite{Draft06} is still rather recent (from 2017) but mature.
%
%We decided to formalize here {\VerSix}, since it is a conservative extension of~{\VerFour}, and the two of them 
%are used in almost the totality of the schemas that we have found.
%
%{\VerNine}, on the other side, is not really a conservative extension, since it adds to {\VerSix} some features 
%that dramatically change the evaluation model.
%First of all, it added two new operators, \xunIts\ and \xunProps, which rely on \emph{annotations} for their 
%semantics, which is a feature that sets them apart from all other operators.
%It also added the operators \xdrecA\ and \xdrRef, which, instead, require a more complex treatment of recursion
%with respect to previous versions, which adopted, instead, a quite standard approach to recursive definitions.
%While it is possible to treat these four operators algebraically, they would much complicate the formal system, 
%hence we decided not to study them here.
%
%However, {\VerNine} also added \xmaxC\ and \xminC\ (see Section~\ref{sec:mincontains}). 
%These two operators are quite interesting for the study of not-elimination and are fully compatible with the {\VerSix} evaluation model, hence we decided to consider them.
%%Finally, it introduced some new syntactic forms, such as \xdepS\ and \xdepR\ instead of \xdeps, which are 
%%elegant and harmless.
%
%%To sum up, in this paper we will formalize {\VerSix} \cite{Draft06}, but we will also study an   extension that includes the new \xmaxC\ and \xminC\ operators.
%%, and, in the surface syntax, we also accept {\VerNine} syntactic variants, such as \xdepS, \xdepR, \xddefs\ for \xdefs, and the presence of other keywords in the same schema object as \xdref.
%\end{toappendix}
%}

%}% hide JSON by example

